Understanding Codebase like a Professional! Human-AI Collaboration for Code Comprehension

Understanding an unfamiliar codebase is an essential task for developers in various scenarios, such as during the onboarding process. Especially when the codebase is large and time is limited, achieving a decent level of comprehension remains challenging for both experienced and novice developers, even with the assistance of LLMs. Existing studies have shown that LLMs often fail to support users in understanding code structures or to provide user-centered, adaptive, and dynamic assistance in real-world settings. To address this, we propose learning from the perspective of a unique role, code auditors, whose work often requires them to quickly familiarize themselves with new code projects on a weekly or even daily basis. To achieve this, we recruited and interviewed 8 code auditing practitioners to understand how they master codebase understanding. We identified four design opportunities for an LLM-based codebase understanding system: supporting cognitive alignment through automated codebase information extraction, decomposition, and representation, as well as reducing manual effort and conversational distraction through interaction design. To validate these four design opportunities, we designed a system prototype, CodeMap, that provides dynamic information extraction and representation aligned with the human cognitive flow and enables interactive switching among hierarchical codebase visualizations. We then conducted a user study with nine experienced developers and six novice developers. Our results demonstrate that CodeMap significantly improved users' perceived intuitiveness, ease of use, and usefulness in supporting code comprehension, while reducing their reliance on reading and interpreting LLM responses by 79% and increasing map usage time by 90% compared to the static visualization analysis tool.

==> Paper/2_related_work.tex <==

\section{Related Work}
\noindent \textbf{Codebase Understanding.} Codebase understanding is a foundational yet challenging task in software development. It often arises when a developer is newly onboarded to a codebase and needs to become familiar with it in order to identify vulnerabilities \cite{xiang2015overview}, make contributions \cite{reefman2024using, hines2023codebase}, or just learn the code \cite{busjahn2013use}. 
Unlike snippet-level code comprehension, codebase understanding emphasizes the architecture, components and their relationships \cite{levy2021understanding}. Traditionally, codebase understanding is aided by static or dynamic analysis tools that generate structural visualizations (e.g., data flows \cite{yin2002program, scitools2025understand, codecompass2018framework, sourcetrail2021explorer, hines2023codebase} and trace graphs \cite{cornelissen2010controlled}). However, these tools are inherently limited by the incompleteness of program analysis and often incur high processing overheads \cite{besset2018sourcetrailue4}. Users also often report steep learning curves and usability challenges \cite{reefman2024using}.


\noindent \textbf{LLM-powered Codebase Understanding.} Recently, LLM-assisted snippet-level code understanding has attracted significant attention, including efforts to explain selected code snippets \cite{andryushchenko2024leveraginglargelanguagemodels,theprogrammersassistant,chen2023gptutorchatgptpoweredprogrammingtool,nam2024usingllmhelpcode,richards2024you} and related concepts \cite{nam2024usingllmhelpcode,andryushchenko2024leveraginglargelanguagemodels}. 
However, limited work have \cite{reefman2024using, berhanu2025ai} explored the application of LLMs for codebase understanding, which is essential in many software engineering scenarios. Reefman et al. \cite{reefman2024using} incorporate the LLM with static‑analysis context (call hierarchies, repository structure, etc.) to answer repository‑scale developer queries.
However, because the system is implemented purely as a chatbot style interface, it lacks designs for human usage in real world.
To address this gap, we adopted a human-centered perspective by examining how code auditors—who frequently onboard to new codebases—develop code comprehension strategies and how these insights can inform system design.

% A closer look at how auditors build an understanding of unfamiliar codebases led us to identify a process we call the “Chain of Understanding”, and their challenges in applying LLMs, and their expectations in LLM assistance. Building on our formative findings, we embed auditors’ “chain-of-understanding” cognitive workflow into an interactive system, \systemabb. The tool provides three new features: (1) alignment with user's natural cognitive flow, (2) hierarchical, interactive visual maps, and (3) expert-oriented guidance. Together, these features let auditors navigate the architecture, explore individual modules, and progressively deepen their comprehension of the codebase.


==> Paper/7_conclusion.tex <==
\section{Conclusion}
This study adopted a human-centered approach to explore how professional code auditors comprehend codebases and how their strategies can inform system design. We proposed four design opportunities for LLM-based systems and implemented \systemabb, a prototype that extracts, decomposes, and visualizes codebase information to support hierarchical understanding. User validation with experienced and novice developers showed that \systemabb enhances intuitiveness, ease of use, and usefulness, while reducing reliance on textual LLM responses. These findings demonstrate the potential of expert-informed, human–AI co-understanding systems to improve large-scale code comprehension and developer onboarding.

\vspace{-8pt}
\section{Data Availability}
\label{sec:data_availability}
All data and code are available on our website \cite{website}. This study has been approved by the Institutional Review Board (IRB) at the authors’ institution.

